Measuring and exploiting the cloud consolidation of the Web

We present measurements showing that the top one million most popular Web domains are reachable within 13ms (in the median) from a collective of just 12 cloud data centers. We explore the consequences of this Web "consolidation", focusing on its potential for speeding up the evolution of the Web. That most popular services reside in or near a small number of data centers implies that new application and transport technologies can be rapidly deployed for these Web services, without the involvement of their operators. We show how this may be achieved by orchestrating a handful of reverse proxies deployed in the same data centers, with new technologies deployed at these proxies being nearly as effective as deploying them directly to the Web servers. We present early measurements of this approach, demonstrating a >50% reduction in Web page load times for users with high latencies to Web servers. We also show that this model, using a small number of proxies, can be surprisingly competitive with extensive CDN deployments, especially in geographies with high last-mile latencies.

==> adoption.tex <==
\section{Adoption of Web delivery tools and protocols}
\label{sec:background}

Various protocols and proposals have been proposed in the past to make Web page delivery efficient. Proposals include tools for compression like WebP~\cite{webp} and GZip, application layer improvements like SPDY~\cite{erman2015towards} and HTTP/$2$~\cite{belshe2015hypertext} and various congestion control mechanisms like BBR~\cite{bbr} and PCC~\cite{dong2015pcc}, to name a few. In this section we measure the adoption rates of WebP and HTTP/$2$ across different countries. For our experiments, we rely on Alexa's~\cite{alexa} top 200 domains per country as available through Amazon ATS~\cite{amazonats}. For 10 countries across globe we load the top 200 Web pages using Google's Lighthouse~\cite{lighthouse} which generates detailed reports on Web pages. We analyze these reports to generate our results.

\begin{figure}
\begin{center}
\includegraphics[width=3in]{figures/webP_comparison.pdf}
\caption{\em The percentage of image bytes wasted per Web page for not having WebP compression varies by $10\%$ in the median across countries for top 200 Web pages. Even for the US, the median percentage of image bytes wasted per Web page is more than $50\%$.}
\label{fig:webp_adoption}
\end{center}
\end{figure}
\parab{Adoption of WebP across countries}
Fig.~\ref{fig:webp_adoption} plots the CDF of the percentage of image bytes wasted per Web page for several countries. The median varies by $10\%$ across $10$ countries. Given the fact that images comprise more than $70\%$ of Web traffic~\cite{agababov2015flywheel}, this variation in adoption across countries is significant. Also, even for the US with the highest WebP adoption rate among the 10 countries, the median percentage of wastage of image bytes is more than $50\%$.

\begin{figure}
\begin{center}
\includegraphics[width=3in]{figures/http2_comparison.pdf}
\caption{\em For top 200 Web pages, the percentage of non-HTTP/$2$ requests per Web page varies by more than $40\%$ across the countries in the $75$-th percentile. The US shows highest HTTP/$2$ adoption.}
\label{fig:http2_adoption}
\end{center}
\end{figure}
\parab{Adoption of HTTP/$2$ across countries}
Fig.~\ref{fig:http2_adoption} plots the CDF of the percentage of non-HTTP/$2$, i.e.\ HTTP/$1$ requests per Web page for several countries. The US shows the best HTTP/$2$ adoption rates and is way ahead of the other countries at higher percentiles. Even for the top 200 Web pages which have a significant fraction of domains in common, at the $75$-th percentile the percentage wastage varies by $40\%$ across countries.

\parab{CGN as an enabler of adoption}
It is easier to make changes at few CGN nodes than millions of Web servers. CGN leverages the fact that Web services are massively consolidated in cloud data centers in order to reach close to them. Hence, effectively CGN nodes are in control of the end-to-end transport between the clients and the Web servers globally. This makes it trivial to test and deploy any new protocol and tool and massively accelerates the adoption of new techniques for Web content delivery. In \S\ref{sec:results} we trivially enable BBR congestion control for clients globally for the 100 Web pages mapped to Azure US WEST 2 data center.

==> background.tex <==
%!TEX root = paper.tex

%\section{Background and related work}

\section{Background \& motivation}
\label{sec:background}

%Content distribution networks build worldwide infrastructures with servers as close as possible to as many Internet users as possible. For instance, Akamai leverages their $233$,$000$$+$ servers located in more than $1600$ networks around the World, to be able to claim~\cite{akamaiInfra}:
%
%{\centering{
%        \hfill
%                \parbox{\columnwidth}{
%                        {\vspace{8pt}
%                                \noindent\emph{``Eighty-five percent of the world's Internet users are within a single `network hop' of an Akamai CDN server.''}
%                                \vspace{-6pt}
%                        }
%                }
%        \hfill
%           }
%}

Content distribution networks build worldwide infrastructures to establish proximity between content and users, and thus allow users to reach their services at lower latencies. However, they are far from a catch-all solution for several reasons:

\parab{Content coverage:} Due to their expense, CDNs are estimated to be used by under $10\%$ of the top $32$,$000$ most popular Web sites, with usage dropping with decline in popularity~\cite{gilad2016cdn}. Further, most CDN-enabled Web sites today do not use CDNs for full-site delivery -- often, the initial HTML, as well as any dynamic or personalized content must still be fetched from the content originator's servers, which could incur a large latency. 

\parab{Last-mile latency:} Last-mile latencies in many parts of the World are extremely poor. For instance, in Pakistan, last-mile latencies for $3$ out of $5$ measured providers are around $100$~ms in the median, and average latency to M-Lab servers within the same city exceeds $100$~ms~\cite{awan2015measuring}. While, not strictly last-mile, median latencies to the nearest M-Lab servers are $\sim$$200$~ms in Africa, Asia, South America, and Oceania~\cite{Hoiland-Jorgensen} even though there are several M-Lab servers in most of these geographies. In Asia, even the fastest of $4$ measured CDNs required an average of $1$~sec to deliver a small (latency-bounded) $12$~KB object, compared to under $0.4$~sec in Europe and North America~\cite{CDNcompare}. On mobile networks, last-mile latencies will likely continue to be poor in many parts of the World for several years, as the HSPA/HSPA+ standards have been or are being deployed, with latencies on the order of $100$~ms~\cite{ilyaHSPA}. For users with such large last-mile latencies, even latency to geographically nearby CDN servers can exceed $100$ milliseconds, and the many RTTs needed to fetch Web content from these servers can still add up to large page load times and poor user experience. 

\begin{figure}
\begin{center}
\includegraphics[width=2.6in,clip]{figures/akamaigrowth}
\caption{\em Akamai's extensive, constantly growing footprint.}
\vspace{-10pt}
\label{fig:akamaiGrowth}
\end{center}
\end{figure}

\parab{Complex, expensive infrastructure:} CDN infrastructure is not only large and expensive, but requires a constantly spreading footprint. While such networks do not release information about their growth over time, we were able to gather some (approximate) data points using the ``Internet Wayback Machine''~\cite{waybackMachine} on Akamai's public page disclosing their network's size~\cite{akamaiInfra}. As shown in Fig.~\ref{fig:akamaiGrowth}, on average, Akamai adds $\sim$$3$,$000$ servers~/~month. In the same period, the number of networks to which they connect increased from $1300$$+$ to $1600$$+$. Relatedly, provisioning CDN infrastructure is a challenging problem because of the need to forecast demands to deploy hardware. When provisioning fails to handle content demand, CDNs must redirect users to farther away servers. 

All of the above challenges stem from a fundamental issue: establishing low-latency connectivity covering most users is made difficult and expensive by the spread of users and the diversity of their last-mile connectivity. In contrast, as our measurements show (\S\ref{sec:consolidation}), achieving proximity to most Web servers is extremely easy and cheap. This simple observation motivates us to explore an ``upside-down'' model of Web page delivery, whereby users establish points of presence near Web servers, and leverage these to fetch content from them using aggressive transport protocols, ideally incurring just one (potentially long) RTT to such a point of presence, together with the much smaller time it takes from there to fetch the Web content from the Web servers (likely incurring many, but extremely short RTTs). Not only is this approach performant (\S\ref{sec:results}), it is also easy to deploy and maintain -- in comparison to building and expanding physical CDN infrastructure, it is rather trivial to provision its (virtual) footprint within public data centers, and to scale it up or down in response to demands. While CDNs also provide services besides reducing latency, such as protection against denial-of-service attacks, these can also be offered using cloud infrastructure~\cite{gilad2016cdn}.

%Establishing points of presence close to most of the World's population requires complex and expensive infrastructure. Even Akamai's extensive infrastructure is limited to the bigger cities, leaving rural and under-developed regions still far from their nearest CDN servers.

%Thus, while CDNs do improve latency for many users and services, they are not a catch-all solution. To address the above problems, we shall explore a dramatically different model: establishing global points of presence on behalf of users, near content servers. In our proposed model, while users will indeed see larger latencies to these more limited points of presence, they will be able to obtain content from them in fewer (ideally, one) round-trips, using aggressive transport protocols. Our proposed design (\S\ref{subsec:details}) requires no changes at Web servers or to Internet infrastructure, only small software changes at user devices. Thus, any user wanting to obtain faster access to any Web service will be able to use our design, irrespective of whether the Web service uses a CDN or not, or if latency to CDN servers from the user's location is small or not.

We thus explore the potential of this upside-down approach as an alternative to CDNs, and in what contexts it can outperform or match CDN-based delivery. We focus on Web page loads, which involve a small amount of latency-sensitive data; for other services like movie streaming, CDNs also help by reducing expensive wide-area bandwidth utilization.



==> design.tex <==
 %!TEX root = paper.tex

\begin{figure*}
\begin{center}
\includegraphics[width=5in]{figures/cloudispproposal.pdf}
\caption{\em The many long client-server RTTs in the default case are replaced by few (ideally, one, with enough available bandwidth) long RTTs between the client and the CGN node, plus many short RTTs between the CGN node and the Web server.\vspace{-10pt}}
\label{fig:cloudbasedisp}
\end{center}
\end{figure*}

\section{A Content Gathering Network}
\label{sec:cgn}

We propose to exploit the proximity of cloud-hosted nodes to most Web servers to build a content gathering network (CGN), so that users are able to get Web content faster. Our approach is illustrated in Fig.~\ref{fig:cloudbasedisp}. The client proxies its Web requests through a CGN node close to the target Web server. This node can obtain content from the server over a small network RTT, and then transmit it to the client using aggressive transport protocols. In the following, we add details to this high-level sketch:

\parab{Client local mapping:} A client needs to map any target Web service to the CGN node closest to the service. This mapping is a small file (few MB), which the client obtains from the CGN. Given the stability of the latencies between Web servers and their mapped CGN nodes (\S\ref{subsec:stableMapping}), measurements, computations, transfers, and updates of these mappings are all infrequent (\eg once a day). In the rare case that mappings are out of date (indicating that the Web service has migrated to a different data center, or its replica in the mapped location is slow or unavailable), there is a performance penalty, but the content can still be obtained -- the CGN node simply fetches it like any other device on the Internet.

\parab{Client-side software:} \debopam{Our current implementation uses a small piece of software running on the client, which the browser uses as a local proxy through standard configuration mechanisms. In this realization, the local proxy maps Web services to CGN nodes. %and uses custom transport protocols to communicate with CGN nodes. 
It forwards Web requests to the CGN node, and as content is received from the CGN node, it serves the content to the browser, which starts loading the page. Standard transport layer optimizations like larger TCP window sizes~\cite{nanditaWindowSize} and persistent connections~\cite{TCPfastopen} are used between the local proxy and the CGN node. At its simplest, the client only needs a browser extension for popular browsers.}


%At its simplest, the client only needs a browser extension for popular browsers. This extension maps each request to a CGN node, and manipulates the browser's proxy configuration to point to the mapped CGN node. This is perhaps the most user-accessible and maintainable solution, and can still obtain substantial benefits (\S\ref{subsec:transport}). 
%If greater control on transport is desired, this may be implemented in a small piece of software running on the client, which the browser uses as a local proxy through standard configuration mechanisms. In this realization, the local proxy maps Web services to CGN nodes, and uses custom transport protocols to communicate with CGN nodes. It forwards Web requests to the CGN node, and as content is received from the CGN node, it serves the content to the browser, which starts loading the page. Our current implementation uses this approach to evaluate the use of UDT~\cite{udtTransport}, TCP Fast Open, and large TCP initial window sizes.

\parab{CGN node:} Each CGN node runs in a cloud data center, and maintains a pool of headless browsers (presently \texttt{PhantomJS}~\cite{phantomjsrelease}) to which incoming client requests are assigned. In case of excessive load, new instances may be launched on separate virtual machines, and requests may be spread across these via a load balancer. On receiving a page request, a browser instance fetches it as usual. Any content received is transmitted in parallel to the client, even as the browser processes it. 

CGN nodes also gather latency measurements as noted earlier (\S\ref{subsec:distributionServers}), which are aggregated at one node and processed to construct the CGN-Web-server mapping. Note again that these are small amounts of data.

\ankit{Our goal is not to re-architect proxies, but to develop a simple architecture for deploying and orchestrating the use of a small number of proxies at appropriate locations. We thus focus on a minimal implementation, relying on experience with deployed systems like Google's Flywheel~\cite{agababov2015flywheel} for software engineering issues, such as for cookies and other client-state.}

\parab{HTTPS:} \ankit{Proxy-based architectures fundamentally operate using network middlemen. Even in the case of CDNs, CDN servers are the middlemen, and trust is not truly end-to-end; rather, in a majority of deployments, Web service operators trust CDNs with their private keys~\cite{cdnKeys}. One potential deployment model for CGN would make the same compromise: the client's browser would be split across the CGN nodes and client-side software, sharing a key, which then sets up two SSL connections: client-CGN and CGN-server. The browser vendor may be responsible for managing client trust (just like CDNs manage server-trust today), and multiplexing client browser instances across physical hardware.}

\ankit{One can further ensure that client data is not seen even by the cloud provider, using solutions like mbTLS~\cite{mbTLS}, running over private computing platforms like Intel SGX~\cite{intelSGX}. An even more private deployment is achievable, in which the client retains end-to-end control. However, this does not provide the benefit of multiplexing that a deployment managed by a popular browser provides. This possibility is unrealistically expensive for now, because of the need for dedicated client virtual machines operating as CGN nodes. However, as serverless computing enables more complex functionality with faster initialization, this can be expected to become feasible -- clients would then operate CGN nodes in serverless mode on platforms like Amazon Lambda~\cite{aws_lambda}, only paying for usage when they send requests. A similar approach is already workable for private email~\cite{palkar2017diy}.}
 
%Accommodating secure pages in our design compromises end-to-end semantics that users expect. \debopam{However, existing solutions like \texttt{mbTLS}~\cite{mbTLS}, which ensure secure multi-party communication using private computing platforms like Intel SGX~\cite{intelSGX}, can be readily deployed to mitigate users' privacy concerns. This will ensure protection of user data on top of third-party infrastructure without compromising on throughput. Nevertheless, we believe a solution focused on HTTP would still be welcome, as evidenced by millions of users using existing solutions such as Opera Mini and Google Flywheel. Also, handling personalization and client-side cache is trivial given that the CGN node is simply an extension of the client's browser to the cloud.}


%However, CDNs also represent a similar compromise, with content originators typically sharing their private keys with CDNs\footnote{{\em``Our results reveal that key sharing is extremely common, with a small handful of hosting providers having keys from the majority of the most popular websites.''} --- Cangialosi et al.~\cite{cdnKeys}}. A similar deployment would work for the CGN -- the CGN would then be able to provide secure service for content providers who share keys in this manner, ensuring faster service to their users. However, there may be opportunities for going beyond this approach: we are investigating whether future availability of private computing platforms like Intel SGX~\cite{intelSGX} can mitigate users' privacy concerns, by preventing the CGN from seeing the content of users' Web requests and their responses\footnote{The CGN would still know which domains users interact with, a limitation that appears fundamental to proxy-based architectures, unless coupled with techniques like onion routing~\cite{tor}.} without compromising on latency. In the meanwhile, we believe a solution focused on HTTP would still be welcome, as evidenced by millions of users using existing solutions such as Opera Mini and Google Flywheel. 

%But It is noteworthy that CDNs also compromise on the end-to-end security of Web transactions, with content originators typically sharing their private keys with CDNs~\cite{cdnKeys}. A virtually identical deployment could work for the CGN, with content originators sharing keys with the CGN instead -- the CGN would then only be able to provide secure service for content providers who share keys in this manner.
 
%Ideally, delivering the content from the CGN to the client should be bounded only by bandwidth-based constraints and one RTT. Given that serving Web requests often involves significant interaction between the CDN front-ends and back-end or origin servers~\cite{pujol2014back}, some long RTTs are often incurred even in the CDN model. Thus, if CGN achieves 1 RTT page load times (modulo bandwidth constraints), then perhaps the role of CDNs in Web page delivery can be substantially reduced, or even entirely eliminated. However, our present implementation often does not hit this goal due to the difference in behaviors between client-side browsers and headless browsers at the CGN. Due to this, to prevent many long RTTs to the CGN, we still rely on traditional CDN nodes to serve content from these secondary requests when we can identify the use of a CDN through simple domain name filters\footnote{Possibly, we also benefit to some extent from anycast-based CDNs; teasing out their impact on our results is left to future work.}. But we do not believe that the $1$-RTT goal is unreachable, and are working towards it. 

%The results above show that a majority of popular web servers are reachable within less than $5$ ms from merely $14$ EC2 instances distributed globally. The mapping between the web servers and the EC2 instances is stable in general which makes it trivial to identify the EC2 instance nearest to a web server. These interesting findings motivate us to explore the possibility of a Content Gathering Network (CGN) which might challenge the existing CDN model of web content delivery. The proposed system, as depicted in Figure~\ref{fig:cloudbasedisp}, comprises of 2 entities: the CGN-node installed in the cloud infrastructure which works on behalf of the client and the client. The client is a HTTP proxy service running at the end user's host. The browser is configured to forward all HTTP requests to the client. On receiving a request to load a webpage, the client forwards the request to the CGN-node which is nearest to the corresponding web server using a persistent TCP connection with large window size. The CGN-node runs a headless browser instance which starts loading the web page by fetching all associated contents from the web server. As the web content is downloaded by the headless browser running in the CGN-node from the server, the CGN-node starts to forward the content to the client in parallel using a TCP byte stream. The client, in turn, serves the content to the browser which starts loading the webpage.\\ 

%Instead of multiple long round trips between the clients and web servers (median is $275.8$ ms from Lahore), we have one long round trip between the client and the CGN-node in the ideal case and multiple very short round trips (median is $4.8$ ms for top $10$,$000$ domains) between the CGN-node and the servers. Nevertheless, in practice we observe more than one round trips between the client and the CGN-nodef primarily because of the difference in behaviors of the client-side browsers and the headless browsers running at the CGN-node. To reduce this overhead, each CGN-node has a light-weight module which can fetch simple contents like individual images, javascripts, etc. directly from the server, bypassing the headless browser altogether. In order to hide the latency due to multiple round trips, we apply a strategy similar to the one used by popular browsers. We use multiple parallel connections between the client and the CGN-node so that additional requests can be sent in parallel.


==> discussion_bckp.tex <==
 %!TEX root = paper.tex

\pagebreak
\section{Discussion topics} \label{discussions}

The CGN model we propose is a significant departure from how Web page delivery works today. Apart from the ``who pays'' question addressed above, we invite discussion and feedback on several topics:
%We thus expect this work to generate significant discussion, including along some of the following topics:

%\parab{Who bears the cost?} While we believe users stuck with poor connectivity would be willing to pay the minimal costs (\S\ref{cost}), this would perhaps be undesirable, in that it shifts responsibility from the content-provider and CDN eco-system onto users. Several alternative models could work: (a) competing cloud providers may bear the cost to attract more Web service providers, promising lower latency access for their users; (b) browser vendors competing for market share could run the service; (c) Web service providers themselves may incur the expense.

\parab{C\textbf{G}N v. C\textbf{D}N:} We believe the CGN model presents different trade-offs than the CDN model -- instead of CDNs operating hundreds of thousands of servers across thousands of locations, perhaps similar or even better performance can be achieved with a CGN. For entirely static content, if CDNs were to use similarly aggressive transport protocols, the latency difference would come down to the CGN-client latency v. CDN-client latency, and the latter would typically be smaller. 
However, for dynamic content, CDNs often need connectivity to the back-end or content-origin servers~\cite{pujol2014back}, ameliorating their client proximity advantage in this comparison. The substantially higher cost and complexity of CDNs thus may not be worth the expense (for low-traffic-volume applications like Web page delivery).

\parab{A matter of time?} If Web servers and CDNs do deploy aggressive protocol enhancements, the CGN approach could lose its utility. However, as pointed out earlier (\S\ref{sec:related}) even the most popular Web servers are slow to adopt enhancements, even when they are backed by industry giants. Further, servers are often conservative in their resource-use per user (to protect against DoS), while our design could potentially create more accountability at the user end, and can thus afford to be less conservative.

\parab{Security, HTTPS:} We do not foresee significant challenges in supporting HTTPS, but the client browser needs to trust the CGN instead of treating it as an eavesdropper, because the CGN node would need to act as a TLS/SSL proxy. Note than CDNs already operate under a similar trust model. There is also scope for using techniques like Intel SGX~\cite{intelSGX} to hide the \emph{content} of client-server interactions from the CGN nodes as a privacy enhancement, although CGN nodes will still be able to see \emph{which servers} a client connects to. CGN nodes would also need effective sandboxing of user requests from each other. We note that CDNs also provide security services like DDoS protection. However, there is no reason cloud infrastructure cannot do the same.

\parab{Fairness:} The use of aggressive transport protocols raises issues of fairness to Internet hosts not using them. However, short flows like those for Web page delivery are inherently disadvantaged in comparison to longer-lived traffic for applications like video streaming. Further, Web browsers already break flow-fairness by employing multiple parallel TCP connections. Nevertheless, we plan to study the fairness-performance trade-off in greater depth in future work.

%\parab{Further optimizations:} The CGN-nodes do not currently cache web content. The latency to fetch popular content can be reduced further if the CGN-nodes cache content following the caching policy specified by the servers. Caching has been deliberately avoided to present the baseline latency improvements for webpages. As more and more users start using the CGN with caching enabled, webpage load times are expected to reduce further. The CGN-nodes can be further optimized by pre-populating the DNS cache and maintaining a pool of connections to popular web servers. CGN-nodes are statically mapped to web servers and hence these pre-population and pre-connection are trivial. Nevertheless, these optimizations are not expected to improve latencies significantly for a system working at scale.\\

%We do not foresee any major challenge in supporting HTTPS traffic. The browser needs to trust the service and do not mark it as man-in-the-middle in order to make it work. Nevertheless, like Google's Flywheel implementation, we have avoided supporting HTTPS traffic in our experiments.\\

%We aim to push the daemons as near to the web servers as possible. In the limiting case, the web servers and the daemons might be co-located in the same physical machine. A round-trip time of zero will further reduce the latency. Nevertheless, the success of this model depends on a very high adoption rate of cloud services by the hosting web servers and the active involvement of cloud service providers in the co-location process. \\

%The cost of this service per user per month is low as discussed in sub-section \ref{cost} and there can be end users in developing countries who want to pay this additional monthly fee to reduce web page load times instead of upgrading their monthly plan. Nevertheless, we strongly believe that the end users should not be charged for reduced latency. Hence we expect a business model in which a cloud provider sells this service to browsers. The providers can benefit from the additional knowledge of the physical resources in the cloud datacenters and can optimize these resources further in order to maximize their profit. On the other hand, the browsers who compete for user base in the emerging markets with high Internet usage can be interested in using such a service by paying a low cost to the cloud providers. Another implicit benefit of this model is that the cloud-based ISP will be fully transparent to the end users.


==> evaluation_bckp.tex <==
 %!TEX root = paper.tex

\section{Evaluation}
\label{sec:results}

We evaluate Web page performance with the CGN across different network regimes. We pick a set of Web sites that are reachable within $10$~ms latency from one cloud data center, within which we run all our experiments. \debopam{We setup both the CGN node and the client within the same data center. This simplifies the experimental setup greatly and minimizes costs for our experiments, while at the same time allowing us to control latency and bandwidth between entities using the standard Linux \texttt{tc}~\cite{tcCommand} tool}. This approach also removes any potential inaccuracies from record-and-replay based experimental methods -- in each case, we are measuring Web pages as they are served live by the Web ecosystem, with our CGN intermediary, and without (henceforth, ``default''). Our clients run the Firefox browser on Ubuntu virtual machines with $2$ cores and $8$~GB memory. The CGN nodes are run on VMs with $4$ cores and $16$~GB memory and use \texttt{PhantomJS}~\cite{phantomjsrelease} as the headless browser. Our current experiments only test HTTP Web sites. For automating Web page loads and recording page load times and related metrics, we use \texttt{sitespeed.io}~\cite{sitespeedio}.

\subsection{Performance metrics}
\label{subsec:metrics}

\begin{figure}
\begin{center}
\includegraphics[width=3in]{figures/metric_comparison.pdf}
\caption{\em A summary of the metrics we tested: while the trends for CGN's improvement in various metrics as client-server RTT increases are broadly similar, user-focused metrics like $85\%$ visual completion time show greater improvement.\vspace{-10pt}}
\label{fig:results:metrics}
\end{center}
\end{figure}

The measurement of Web page performance is continually evolving, so we test a broad range of metrics, including page load time (Load time, based on \texttt{OnLoad}); time for $85\%$ visual completion (viz$85$, indicative of when most of the visual content is populated); first paint time (when the first content is displayed on the browser);  last visual change (beyond which there are no visual changes, although resources such as scripts may continue to load); and two varieties of ``speed index'' (measuring progression of the page load; lower values implying that most content was loaded early) --- one based on visual changes (Speed Index) and another based on when different resources are loaded (RUM Speed Index). While the absolute values of these metrics vary broadly, looking at \emph{improvement} between the default page fetches and page fetches using our approach across different metrics simplifies the picture greatly.

We illustrate such percentage improvement in various metrics with CGN compared to default page loads without any intervening proxy, using one representative example from our results. (Other details for this result shall follow in \S\ref{subsec:speedup}.) Fig.~\ref{fig:results:metrics} shows the percentage decrease in each metric using the CGN (higher values imply that CGN improved the metric by a larger amount). The two speed index variants gave near-identical results, and are shown together as ``Speed Index''. The three metrics that prioritize early parts of the page load (first paint, viz$85$, and Speed Index) exhibit very similar behavior, showing greater improvement than page load time and last visual change, both of which place greater focus on completion. All metrics show greater improvement for scenarios where the network RTT is larger, as expected by virtue of our design. A manual inspection of our traces revealed that most content loaded later is advertising related. Given this, and (relatedly) the increasing importance placed on such user-focused metrics, for the rest of our analysis, we only show results on viz$85$ time. Nevertheless, we note that our current implementation does not prioritize any type of resources over others (\eg images over script, or vice versa), sending resources to the client as they are received by the CGN. Approaches optimizing the order and timing of delivery~\cite{shandian, polaris, vroom} to speed up desired target metrics may be incorporated into our design, and may provide additional benefit. However, we leave a quantification of this to future work.

\subsection{Faster pages with CGN}
\label{subsec:speedup}

\begin{figure}
\begin{center}
\includegraphics[width=3in]{figures/cgnBetterIncrLatency.pdf}
\caption{\em With bandwidth fixed at $10$~Mbps, as client-server latency increases, the default case shows a very large linear increase in viz$85$ time. Using CGN, the dependence on the network RTT is substantially reduced, resulting in a large improvement for clients with large latency to the server.\vspace{-10pt}}
\label{fig:results:increasingLatency}
\end{center}
\end{figure}

We test the $100$ most popular sites, servers for which are within $10$~ms from our cloud-based virtual client. We fetch these pages without any interposing proxy (the default case) and using a CGN node in the same data center, \debopam{and perform these tests while varying bandwidth and latency between the client and the CGN node.}%($\in \{2, 5, 10, 20\}$~Mbps), as well as adding increasing amounts of latency ($\in \{20, 40, 80, 160, 320\}$~ms) for all outgoing traffic at the client. 

%\begin{figure}
%\begin{center}
%\includegraphics[width=\linewidth]{figures/cgnBetterIncrBandwidth.pdf}
%\caption{\em With client-server latency fixed at $160$~ms, as bandwidth increases, viz$85$ does not show a large improvement for CGN, but in the default case, there is a substantial reduction going from $2$~Mbps to $10$~Mbps.}
%\label{fig:results:increasingBandwidth}
%\end{center}
%\end{figure}

Fig.~\ref{fig:results:increasingLatency} shows results for median viz$85$ time across the $100$ pages, with increasing latency, with bandwidth remaining fixed at $10$~Mbps. Results for other bandwidth settings show similar trends. In the default case, as the network RTT increases, viz$85$ time shows a large linear increase. In contrast, the CGN effectively decouples (to a large extent) this dependence, showing much smaller increases in viz$85$ time. For clients with $160$~ms latency to the Web server, the CGN loads pages $55\%$ ($4.2$~s) faster. Thus, for clients with poor last mile latencies, and other clients that are distant from their target Web servers, our simple approach yields a large advantage. \debopam{We observed that bandwidth plays a much more limited role (in line with expectations, hence results excluded) in Web page performance beyond a few Mbps.}

%Fig.~\ref{fig:results:increasingBandwidth} shows results with increasing bandwidth, with additional client-server latency remaining fixed at $160$~ms. As is clear from the contrast with Fig.~\ref{fig:results:increasingLatency}, bandwidth plays a much more limited role (in line with expectations) in Web page performance beyond a few Mbps, while network RTT continues to have a linear impact. At low bandwidth, we observe that the client blocks for longer on resources from the network in the default case, leading to a larger performance gap. In effect, CGN thus provides dependency resolution~\cite{polaris,vroom} without any Web page or server modifications.

%\begin{figure}[tb]
%\begin{center}
%\includegraphics[width=\linewidth]{figures/top_plt.pdf}
%\caption{\em PLTs from Lahore for the top $100$ domains which map to North California or Frankfurt.}
%\label{fig:webPLTtop}
%\end{center}
%\end{figure}
%
%\begin{figure}[tb]
%\begin{center}
%\includegraphics[width=\linewidth]{figures/rand_plt.pdf}
%\caption{\em PLTs from Lahore for $100$ random domains which map to North California or Frankfurt.}
%\label{fig:webPLTrand}
%\end{center}
%\end{figure}


%\begin{figure}[tb]
%\begin{center}
%\includegraphics[width=\linewidth]{figures/comparison_flywheel.pdf}
%\caption{\em PLTs from Lahore for the top $30$ domains which map to NC or Frankfurt, with CGN, with Flywheel, and with neither.}
%\label{fig:flywheelCompare}
%\end{center}
%\end{figure}

%\subsection{Optimizing transport} 
%\label{subsec:transport}

%CGN's design, with software at the client and at the CGN cooperating for the long-RTT data transfer, allows us to experiment with different transport layer protocols between the client and the CGN. We ran experiments using UDT~\cite{gu2007udt}, TCP Fast Open~\cite{TCPfastopen} (with an initial congestion window of $10$) and persistent TCP connections, whereby the congestion window size is persisted across connections between the same CGN proxy and the client. Note that in most cases, our interest is in sending data from the CGN node to the client. However, to avoid additional state at the CGN, the initial window size from the CGN to the client can be persisted by the client storing this information, and sending it to the CGN node with a new request (for instance, by advertising a receive window equal to this stored value, or by including it in the TCP Fast Open cookie). 

%\begin{figure}
%\begin{center}
%\includegraphics[width=\linewidth]{figures/protocolComparison_Viz85.pdf}
%\caption{\em Performance of the CGN varies with the transport protocol used between the client and the CGN with bandwidth fixed at $10$~Mbps.}
%\label{fig:proto_comp}
%\end{center}
%\end{figure}

%Fig.~\ref{fig:proto_comp} shows median viz$85$ times (across our test set of $100$ pages) for the default page fetch (without CGN, and with the default Linux TCP stack with initial window size of $10$) and for CGN with the three transport variants discussed above, as client-server latency increases. While UDT only provides a small advantage (particularly in relative terms at higher RTTs), CGN with TCP Fast Open and persistent TCP show a large performance improvement over the default page fetch. While there is also an $18$-$30\%$ viz$85$ reduction going from TCPFO to additionally persisting the window size for larger RTTs, most of the benefits of the CGN over the default page fetch can be obtained using TCP Fast Open, and thus would be attainable with simple client-side software changes through a browser extension. At a latency of $160$ms, the reduction in viz$85$ is $54$\% with TCP Fast Open while that with persistent TCP is $64$\%. These results were collected without bandwidth restrictions; results with more limited bandwidth reduce the additional advantage from persisting window sizes, but leave the rest of the comparison similar. All other results in the paper use the persistent TCP connections.

\subsection{CGN is faster than Flywheel} 
\label{subsec:flywheel}

\begin{figure}
\begin{center}
\includegraphics[width=3in]{figures/flywheelComparison.pdf}
\caption{\em CGN improves viz$85$ by $58\%$ in the median compared to Flywheel in tests across $100$ pages with $2$~Mbps bandwidth and $160$~ms of additional latency at the client.\vspace{-10pt}}
\label{fig:results:flywheel}
\end{center}
\end{figure}

We compare CGN to Google's Flywheel system~\cite{agababov2015flywheel}. While Flywheel is targeted at mobile devices, the same functionality is also made available by Google for the desktop Chrome browser in the form of the ``Data Saver'' extension~\cite{datasaver}. These experiments thus use the Chrome browser to fetch the same $100$ Web pages as before with the CGN, or with Flywheel, or with neither, with a fixed network RTT and increasing bandwidth at the client. Flywheel, being a compression proxy, is most advantageous in low-bandwidth settings, so we only include results for a client with $2$~Mbps bandwidth; comparisons with higher bandwidth are more favorable to CGN.

Fig.~\ref{fig:results:flywheel} shows that CGN achieves a substantial performance advantage over Flywheel, which does not improve performance much beyond the default. This is in line with results reported by Flywheel authors, indicating that while Flywheel is extremely effective at meeting its goal of conserving bandwidth, results on latency improvement are mixed, with small improvements or negligible degradation in performance in most cases. Compared to Flywheel, CGN achieves a $53\%$ reduction in the median $85\%$ visual completion time.

%Note that our design does not incorporate Flywheel's compression and prefetch optimizations; neither does it have the benefit of a Google-like infrastructure. 
We also tested a variant of CGN with WebP compression for images (like Flywheel) using the webp-imageio library~\cite{imageio}. We first loaded several pages with and without Flywheel, storing their default images and Flywheel's WebP versions of the same images, and set parameters for our compression to match Flywheel's resulting images. However, as Fig.~\ref{fig:results:flywheel} shows, compression deteriorated the performance of CGN by $27\%$ in the median. We find that on-the-fly WebP compression incurs a significant amount of compute time on the critical path and eliminates any advantage from the resulting faster transfers of compressed images. \debopam{Nevertheless, the CGN variant with compression remains $46\%$ faster in the median than Flywheel.}
%One caveat to our analysis is that we did not investigate possibilities for speeding up the compression. It is also likely that in a practical deployment, such compression is a one-time cost and results are cached at least for the most popular pages, but this is difficult to quantify precisely for CGN, as it depends on access patterns. Nevertheless, the CGN variant with compression remains $46\%$ faster than Flywheel, thus achieving both speed and reduction in bytes transferred.
%Note that like Flywheel, even a small performance degradation (of in the case of CGN, slightly less improvement over the default) for adding compression may be acceptable to some clients.

\subsection{Single proxy solutions fall short} 
\label{subsec:oneproxy}

\begin{figure}
\begin{center}
\includegraphics[width=3in]{figures/client_to_proxy_lat_0.pdf}
\caption{\em A single proxy near the client results in poorer performance for content that is far away. The intuition for this is evident in Fig.~\ref{fig:cloudbasedisp}: an edge proxy still incurs many long RTTs to the Web server, which CGN minimizes.\vspace{-10pt}}
\label{fig:any_proxy_model}
\end{center}
\end{figure}

Several recent proposals have examined proxy-based architectures (\S\ref{sec:related}). However, any solution based on a single proxy will incur several long RTTs between the proxy and far away Web servers. Further, \emph{if} a single proxy is deployed, the best location is at the edge, near the client (to avoid instances of ``hair-pinning'', whereby, requests first go towards the proxy, but then need to be fulfilled using resources in the opposite direction with respect to the client). In contrast, CGN functions using several distributed proxies, directing clients to a CGN node which typically achieves a latency of $\sim$$10$~ms to the target Web server. We compare these two alternatives in a simplified setup. Suppose the client-server latency is $x$~ms, and CGN and the proxy are both on the client-server path (such that using either does not add additional latency). For an ``edge proxy'', the client-proxy latency is, ideally, nearly zero, with the entirety of $x$ being proxy-server latency. For CGN, typically, the CGN-server latency is negligible, with nearly the entirety of $x$ being client-CGN latency. Thus, we compare the two approaches as $x$ varies, with $x$ being the proxy-server latency in the edge proxy design, and client-CGN latency using CGN. Note that achieving near-zero client-proxy latency is virtually impossible for large fractions of the World's population with poor last-mile latency (\S\ref{sec:background}), so this comparison is generous to the edge-proxy approach in those settings. We simply use the CGN itself as the edge proxy, with this experiment serving the goal of illustrating the importance of CGN's proximity to Web servers.

Fig.~\ref{fig:any_proxy_model} shows that in line with expectations, at small client-server latencies, placement near the client or near the server is similar, with all latencies involved being small. However, as the client-server latency increases, CGN's placement near the Web server becomes crucial to achieving higher performance. Even when the client-server latency is merely $40$~ms, CGN achieves $30\%$ lower viz$85$, with this advantage increasing with client-server latency to $54\%$ at $320$~ms. We acknowledge that other recent work has qualitatively (but not quantitatively) made a similar observation, recommending that ideally, their proxies be deployed as reverse proxies co-located with the Web server~\cite{shandian}. Our measurements in \S\ref{sec:consolidation} and our analysis of load time improvements reveal the ease of deploying such an architecture independent of Web service providers, and its benefits.





==> modeling_bckp.tex <==
 %!TEX root = paper.tex

\section{CDN-free Web page delivery?}
\label{subsec:cgnCDN}

\begin{figure}
\begin{center}
\includegraphics[width=3in]{figures/cdn_modelling_viz85_ws_160.pdf}
\caption{\em With client-server latency set to $160$~ms, we emulate results for $3$ possible uses of a CDN, under increasing client-CDN latency: with the CDN only serving all images; serving a random $90\%$ of requests; and serving all requests.\vspace{-10pt}}
\label{fig:cdn_model}
\end{center}
\end{figure}

Our results comparing CGN-based Web page delivery to the default show substantial performance improvements. However, these results were obtained by adding additional latency to all requests from a client to emulate large client-server latency. In a CDN-supported Web service, this is not a realistic comparison -- CDNs make extensive efforts to place their servers closer to clients, and resources fetched from CDNs may thus be delivered over much smaller RTTs. We next explore how fetching Web pages using CGN compares to fetching pages supported by a CDN.

We emulate different extents of CDN-support: (a) fetching only images through a CDN\footnote{Images comprised $74\%$ of the bytes in pages served by Flywheel's deployment~\cite{agababov2015flywheel}, so this is the byte-dominant part of Web pages.}; (b) fulfilling a random $90\%$ of requests through a CDN; and (c) fulfilling all requests through a CDN. The rationale for evaluating options (a) and (b) stems from our conversations with a large CDN operator, which indicate that most of their customers do not use their services for full-site delivery, rather offloading only parts of it. For these experiments, we add different amounts to latency to requests fulfilled through the CDN (in accordance with the three above options) and to other requests, thus modeling smaller client-CDN latency and a larger client-server latency.

Results in Fig.~\ref{fig:cdn_model} show the dependence of $85\%$ visual completion time on the client-CDN latency (with client-server latency fixed to $160$~ms). In line with expectations, the more the content served through the CDN, the better the performance. However, as the client-CDN latency increases, performance degrades quickly. In contrast, as observed earlier, the CGN effectively reduces the dependence on the network RTT, thus gaining an advantage when the RTTs are larger -- even at a client-CDN latency of $80$~ms, CGN is $24\%$ faster. Thus, particularly for users with large last-mile latency, CGN would continue to have a performance advantage over CDN-based delivery. 

A caveat to these results is that they do not account for the possibility that CDNs, like the CGN, themselves may push towards delivering objects in a single RTT (modulo bandwidth constraints) -- for instance, the ``All requests'' result in Fig.~\ref{fig:cdn_model} is the same as the default case in Fig.~\ref{fig:results:increasingLatency}. While some of these Web pages are indeed fetching some resources from CDNs, and thus benefiting from the optimizations CDNs today do, this is clearly inadequate to fully assess the strength of CDN-based Web page delivery. It should be obvious that \emph{if} a CDN performs full-site delivery, and uses the \emph{same} optimizations as a proxy (for both networking and resource prioritization), then it will outperform the proxy, by virtue of incurring a shorter RTT. CDNs do use more aggressive transport than most Web servers, with some using congestion window sizes as large as $46$ packets~\cite{cdnInitWindow} compared to the Linux default of $10$. Unfortunately, a negligible fraction of the pages tested use CDNs extensively. Thus, in the following we use our experimental data to build a simple model to explore this scenario and estimate the CDN's advantage.

%\begin{figure}
%\begin{center}
%\includegraphics[width=\linewidth]{data/no_cgn_cdn_modelling/no_cgn_cdn_bw_10.pdf}
%\caption{\em No CDN/CGN modelling - bw 10Mbit}
%\label{fig:no_cdn_cgn_model}
%\end{center}
%\end{figure}

We construct a simple, linear model of how the involved round-trip latencies --- client-server ($RTT_s$), client-CGN ($RTT_g$) and client-CDN ($RTT_{lm}$) --- impact Web performance using CDNs and the CGN. For simplification, drawing on our measurements, we assume that CGN-server latency is nearly zero, \ie $RTT_g = RTT_s$. We also assume that enough bandwidth is available -- in our experiments, beyond a few Mbps, bandwidth changes only had a small impact on performance. We use the $10$~Mbps data to build our model.

Using the data in Fig.~\ref{fig:results:increasingLatency} and Fig.~\ref{fig:cdn_model}, we compute regression-based best-fit lines for viz$85$ for default page loads ($t_{D}$) and CGN-supported Web page loads ($t_{CGN}$):
\begin{align}
t_{Default} & = 36.4 * RTT_{s} + 2.1   \\
t_{CGN}     & = 3.8 * RTT_{s} + 2.7 
\end{align}

Thus, as noted in our discussion of the experimental results, CGN depends much less on network RTT (less than $4\times$) than the default ($36\times$). However, the addition of an on-path proxy seems to incur some additional overhead in the form of the larger constant for CGN ($2.7$~seconds vs. $2.1$ for default). Based on this network vs. compute breakdown, we can construct two additional hypotheticals -- a well-tuned CGN with near-zero processing overhead (CGN\textsuperscript{*}), and a well-tuned CDN with CGN-like dependence on the network (CDN\textsuperscript{*}) as follows:
\begin{align}
t_{CDN^*}   & = 3.8 * RTT_{lm} + 2.1   \\
t_{CGN^*}   & = 3.8 * RTT_{s} + 2.1
\end{align}

Note that CGN\textsuperscript{*} incurs $RTT_{s} > RTT_{lm}$, where $RTT_{lm}$ is the last-mile latency, which the CDN observes. Suppose $RTT_{s} = \Delta + RTT_{lm}$ for some $\Delta > 0$. We can then estimate the performance of the CDN and CGN using this model across different values of $RTT_{lm}$ and $\Delta$. Fig.~\ref{fig:cdnVcgnIdeal} shows these estimates for CGN (normalized to performance as measured from the Web ecosystem today), and for CGN\textsuperscript{*} (normalized to estimated performance for CDN\textsuperscript{*}). As our experimental results already showed, CGN achieves substantial performance benefits over default page fetches today (with normalized performance values under $1$). Further, this advantage improves as last mile latency increases. 

Of greater interest here, is the comparison to an ideal CDN\textsuperscript{*}. As noted above, CGN\textsuperscript{*} will achieve performance lower than CDN\textsuperscript{*}, but the difference is not very large. In particular, for small $\Delta$, performance is roughly $5\%$ worse than CDN\textsuperscript{*}. Note that a small $\Delta$ can be easy to achieve with relatively little replication (effectively, ``CDN-lite''), because it does not require presence at the edge. Further, performance relative to CDN\textsuperscript{*} improves (\ie becomes closer to $1$ in the Fig.~\ref{fig:cdnVcgnIdeal}) as the last-mile latency increases -- in such regimes, the advantage of CDN\textsuperscript{*} is reduced by the last-mile latency forming a larger fraction of the client-server RTT. Lastly, note that this model assumes the CDN does not incur any round-trips to the server; which is unlikely to be the case for dynamic, personalized content. Thus, a simple design based on a small number of worldwide sites can effectively compete not only with today's Web ecosystem, but also with a well-tuned CDN doing full-site delivery and employing aggressive network optimization.

%In summary, a simple design based on our observation of server consolidation in the cloud has the potential to nearly match the performance of a well-tuned CDN doing full-site delivery and employing aggressive network optimization. We acknowledge that as compute and network bottlenecks shift with page load optimization through server-client interaction~\cite{vroom} or more sophisticated split-browser architectures~\cite{shandian}, this analysis will require adjustment. Nevertheless, our results indicate that if a CGN-like service is widely deployed (\eg as part of popular browser platforms, thus covering most clients), it could substantially diminish or eliminate the incentives for maintaining CDN reach beyond a small number of sites, and extend CDN-like performance to the vast majority of services that do not use them today.

%\begin{figure}
%\begin{center}
%\includegraphics[width=\linewidth]{figures/cdnVcgnToday}
%\caption{\em As last-mile latency dominates, CGNs advantage over CDN-based delivery grows.}
%\label{fig:cdnVcgnToday}
%\end{center}
%\end{figure}

\begin{figure}[t]
\begin{center}
\includegraphics[width=3in]{figures/cdnVcgn}
\vspace{-12pt}
\caption{\em As last-mile latency dominates, the difference between an ideal CDN and CGN diminishes.\vspace{-10pt}}
\label{fig:cdnVcgnIdeal}
\end{center}
\end{figure}
%
%\begin{figure}
%\begin{center}
%\includegraphics[width=\linewidth]{data/bypass_nobypass/bypass_nobypass.pdf}
%\caption{\em Performance comparison - bypass vs. no-bypass}
%\label{fig:bypass_nobypass}
%\end{center}
%\end{figure}

\section{Isn't this very expensive?} 
\label{sec:cost}

\begin{figure}[t]
\begin{center}
\includegraphics[width=3in]{figures/parallelization_lat_160_viz85.pdf}
\caption{\em Performance of CGN with increase in the number of concurrent clients at client-CGN latency of $160$~ms and bandwidth of $10$~Mbps.\vspace{-10pt}}
\label{fig:parallelization}
\end{center}
\end{figure}

%\begin{outline}
%        \1 Refresh the back of envelope: 3000 pages per user; avg. bw cost; first with just 1 request running at CGN at one time.
%        \1 Plot on \# simultaneous clients
%        \1 Modified calculation
%        \1 Mention further opportunities for optimization
%\end{outline}

At first, it may appear that operating such a globally distributed infrastructure on behalf of users could be exorbitantly expensive. However, we find that with multiplexing across potential users of such a service, this need not be the case. In the following, we present a rough analysis of CGN's per user cost.

We find that the average Web page is $\sim$$2$~MB in size, and requires $5.2$~seconds of service time at the CGN, computed as the time from when the CGN receives a request to when it finishes processing for the request. The average costs of compute (with the \texttt{c4.xlarge} instances we used) and networking across EC2 sites are $\$0.232$ per hour and $\$0.115$ per GB~\citep{EC2pricing}. Using an estimate of $3$,$000$ Web pages per month fetched per user~\cite{theNielsenReport}, the monthly costs of network traffic and compute per user are \$$0.66$ and \$$1$ respectively, coming to a total of $\$1.66$ per user per month.

Further, we find that a single \texttt{c4.xlarge} instance can concurrently support several users' requests without much performance degradation. We experimented with varying numbers of clients fetching the same set of $100$ Web pages simultaneously through a single instance, with no caching enabled at the CGN in servicing these requests. Each client also shuffles the order in which it fetches the set of Web pages to avoid any additional server-side overheads from (near) simultaneous arrival of these requests. As Fig.~\ref{fig:parallelization} shows, performance does not deteriorate until $4$ parallel clients (the seeming speedup is within the variance), and shows only minimal degradation for up to $10$ clients. With $10$ concurrent clients, the observed median viz$85$ time using the CGN is still $51\%$ less than that for the default. Adjusting the compute costs using $4$ concurrent clients brings the total cost per user per month down to \$$0.91$.

Admittedly, this cost estimate assumes $100\%$ system utilization, while in practice demand can be expected to be variable over time, necessarily leading to some inefficiencies. Note however, that it is fairly trivial to acquire additional resources to accommodate short-term increases and to release them when demand drops. Further, our estimate is based on an extremely simple, unoptimized proxy, running a full browser, loading each page to completion. Other recent work has already demonstrated that Web proxies can be made much more efficient, \eg by not performing rendering~\cite{shandian}, and not executing all scripts~\cite{proxyEfficient}. Thus, an operational CGN could likely be run at much lower cost than our above estimates.

%A framework like CGN, which is expected to operate globally and serve millions of users, is practical only if the costs of operating the system is low. We found that an average Web page is $2$MB in size and takes $6$s \fixme{verify from CGN modelling} to load at the client when the client is in close proximity of the CGN. According to a recent report~\cite{theNielsenReport}, an average user requests $3$,$000$ pages per month. The average costs of compute (for compute optimized c$4$.xlarge instances) and networking across EC2 sites are respectively $0.232429$/hour $0.114643$/GB according to the latest pricing~\citep{EC2pricing}. Going by the numbers above, the monthly costs of network traffic and compute per user are \$$0.66$ and \$$1.16$ respectively. However, we find that with multiplexing across potential users of such a service, this need not be the case. As shown in Fig.~\ref{fig:parallelization}, the performance of the CGN does not detoriorate for less than $4$ concurrent users. Even with $10$ concurrent users, the observed median viz$85$ using CGN is way below that when CGN is not used. Considering $10$ concurrent users per node, the compute cost reduces to \$$0.11$ per user per month. Hence the cost of operating the CGN is way below a dollar per user per month. As evident, there is a tradeoff between the performance of the CGN and the number of parallel users and the parameters can be tuned according to requirements.


%At first, it may appear that operating such a globally distributed infrastructure on behalf of users could be exorbitantly expensive. However, we find that with multiplexing across potential users of such a service, this need not be the case. For an average request, we find that a CGN node uses $\sim$$300$~ms CPU time and $\sim$$2$~MB network bandwidth in both directions. Suppose that the average user requests $5$,$000$ pages per month\footnote{Most users seem to browse substantially less than this~\cite{theNielsenReport}.}. Conservatively using the highest costs for EC2 nodes\footnote{Reserved \texttt{m4.10xlarge} instances with upfront payment are priciest at Sao Paulo --- \$$1.828$/hour~\cite{EC2pricingSaoPaulo}. Bandwidth costs are \$$0.01$/GB.} leads to a cost estimate of \$$0.934$ per user per month. Even if the system operates at substantially lower efficiency, we believe the costs would be reasonable --- for Lahore, they amount to $\sim$$10\%$ of the cost of typical broadband plans.

%Further, suppose that we pay the highest costs for reserved instances across all locations (\ie \$$1.828$ per hour for each \texttt{m4.10xlarge} at Sao Paulo~\cite{EC2pricingSaoPaulo}) and network traffic costs of USD $0.01$ per GB. Then the cost per user per month is \$$0.934$. Even if the system operates at substantially lower efficiency, we believe the costs would be reasonable --- for Lahore, they amount to $\sim$$10\%$ of the cost of broadband plans. 
%While we believe users stuck with poor connectivity would be willing to pay the minimal costs, this would perhaps be undesirable, in that it shifts responsibility from the content-provider and CDN eco-system onto users. Several alternative models could work: (a) competing cloud providers (Amazon, Azure, Rackspace) may bear the cost to attract more Web service providers to their infrastructure; (b) browser vendors competing for market share could run the service; (c) Web service providers themselves may incur the expense.

%Nevertheless, we hope that other parties than the users (\ie advertisers, browser vendors, Web service providers, etc.) could instead bear the cost of an actual deployment.
%is USD $(1.828*0.5 + 0.01*2)$ or USD $0.934$. Note that network traffic is twice the monthly data usage per user as the content has to be fetched by the CGN-nodes from servers and forwarded to the clients. Even if we assume that the CPU usage is 50\%, the monthly cost per user is no more than USD $(1.828 + 0.02)$ or USD $1.848$. Even in the developing countries, this price is a very small fraction of the monthly ISP charges. In section \ref{discussions} we discuss business models which enables the end users to use this service without spending any money.


 %!TEX root = paper.tex




==> pointsolutions.tex <==
\section{Speeding up the Web using proxies}
\label{sec:pointsolutions}

Given the impact of latency on user experience, there is a large body of work on speeding up the Web. A large fraction of work focuses on using proxy-based solutions to reduce latency as we discuss below.

\parab{Optimizations close to the end user}
Various Web proxy based solutions, which rely on using a well-provisioned proxy node close to the client, exist. Solutions from large browser vendors include Opera's Mini and Turbo~\cite{operamini,operaturbo}, Google's Flywheel~\cite{agababov2015flywheel} and Amazon's Silk~\cite{amazonsilk}. Opera's solution of compressing and rendering Web pages on Mini servers has been recently replaced by Turbo mode~\cite{operanew} - Web content is compressed at the proxy while rendering happens at the client. Google's Flywheel performs various optimizations which include compression, caching, pre-connect (having live connections open to content servers in order to serve client requests) and pre-fetch (pre-fetching Web content to be requested by users). Amazon's Silk is a similar proxy-based solution which relies on analyzing aggregated Web traffic and pre-processing Web pages based on predictive algorithms to deliver content faster. While the above solutions focus on reducing data usage of clients, there exist other proxy-based point solutions focused on low latency Web browsing. WebPro~\cite{sehati2016network} relies on a well-provisioned proxy which maintains a database of resource lists for Web pages and sends requests proactively to the corresponding content servers while serving a client. The proxy is deployed in ``the wired part of the network''. Cumulus~\cite{netravali2015mahimahi} relies on ``a well-provisioned cloud server'' and PARCEL~\cite{parcelSivakumar} relies on a proxy ``implemented on a powerful server''.

\parab{Optimizations close to the Web server} 
Shandian~\cite{shandian} proposes a split-browser architecture for speeding up the page load process. A well-provisioned proxy loads Web pages on behalf of clients and while transferring content to clients prioritize state critical for the page load. Shandian proposes placement of the proxy servers close to the Web servers. Ideally the proxy server has to be co-located with the Web server.

\parab{No clear deployment model}
None of the above proxy-based point solutions have a clear deployment model. While it is hard to scale solutions which rely on placing proxies close to clients, it is not very easy to realize any solution that relies on co-locating reverse proxies with Web servers unless there is a clear deployment model. Making any change at the Web server is an extremely slow process and can take years to get adopted. In this paper, we propose a public cloud based deployment model for these proxy solutions and show that: (a) a small number of cloud proxies suffice, and (b) these can be easily exploited to build an immediately deployable system, without the cooperation of any other parties than the clients seeking better performance.

==> results.tex <==
 %!TEX root = paper.tex

\section{Results}




==> title.tex <==
 %!TEX root = paper.tex

%make title bold and 14 pt font (Latex default is non-bold, 16 pt)
%\title{\Large \bf I'd Go the Whole Wide World}
%\title{\Large \bf CastNet: Fishing for better Web performance}
\title{\vspace{-.5in}\Large \bf A Cloud-based Content \emph{Gathering} Network}

%for single author (just remove % characters)
\author{
{\rm Debopam Bhattacherjee}\\
ETH Z\"{u}rich
\and
{\rm Muhammad Tirmazi}\\
LUMS
\and
{\rm Ankit Singla}\\
ETH Z\"{u}rich
% copy the following lines to add more authors
% \and
% {\rm Name}\\
%Name Institution
} % end author

\maketitle

